ARTOO-DARTU: Studying AR-HRC With AR Obstruction Mitigation During a Warehouse Task

Human-robot collaboration (HRC) often requires robot intentions and internal states to be conveyed to users for task efficiency and safety. Recently, augmented reality (AR) situated analytics provide such real-time robot feedback in HRC contexts. However, AR situated analytics can obstruct important real-world elements, posing safety and usability risks, especially when content is dynamically positioned relative to movements of mobile robots in a warehouse HRC scenario. In this paper, we introduce the Augmented Reality Technique Of Obstruction Deterrence while Aiding Robotic Teaming for Users (ARTOO-DARTU), an AR system tailored specifically for warehouse HRC that enables real-time robot situated analytics and control while preserving visibility of the real world through an obstruction detection and mitigation pipeline (ODM) that is uniquely suited for AR-HRC. To evaluate ARTOO-DARTU, we developed Pocket MonstARs, a controlled gamified abstraction of HRC warehouse inventory picking in which virtual monsters serve as proxies for pick targets, while labeled and object-marked boxes preserve the real-world identification demands of the picking task. In a 34-participant user study, we found that our designed AR situated analytics yielded a 46% increase in efficiency on the overall HRC task, but only when the ODM was active. Participants with the ODM active were also 61% faster on subtasks requiring visibility of the real world. Our findings demonstrate that, when paired with our developed ODM to prevent real-world obstructions, the situated analytics in ARTOO-DARTU can significantly enhance efficiency and user experience in AR-HRC warehouse scenarios.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sec/system_evaluation.tex <==
\section{System Evaluation}
\label{sec:technicaleval}
In this section, we evaluate \ProjectName by analyzing the situated analytics' update latencies. We also characterize the performance and latency of the \ObsPipeName. 

\subsection{Situated Analytics Latencies}
\label{subsec:aarclatencyandalignment}

% \noindent\textbf{Hololens App Analytics Alignment.}
% To evaluate how well the situated analytics maintain alignment with the TurtleBot when using \ProjectName, a researcher first performed the initial coordinate setup process. The researcher then commanded the TurtleBot to drive away from the alignment location along a straight path, stopping at 4 positions spaced apart at 1.5~m intervals, reaching a maximum distance of 6~m. Meanwhile, the location indicator moved with the TurtleBot. At each position, the researcher placed a virtual rod at the center of the TurtleBot, over which the location indicator would hover in an ideal scenario. The \SystemName then computed the offset from the center of the location indicator to the rod, providing a measurement of the horizontal misalignment of the indicator. This measurement was repeated at each position over 10 trials. The average misalignment was 5$\pm 1.42$, 8$\pm 0.95$, and 14$\pm 2.47$~cm at distances of 1.5, 3, and 4.5~m respectively. As expected, the alignment of the analytics degraded as distance increased. At 6~m away from the alignment location, the misalignment was on average 16$\pm 2.08$~cm, just under the radius of the TurtleBot. However, since the alignment error is near the TurtleBot's size, we find the analytics in practice look well-aligned even when the TurtleBot has moved larger distances from its initial location.
% \noindent\textbf{Location, Trajectory, and Command Indicator Latencies.}
We characterize update latencies of \ProjectName's location and trajectory indicators and the latency for the TurtleBot to respond to a command from the \SystemName. We performed the measurements with all of \ProjectName active, including all indicators and the \ObsPipeName. To collect measurements, a researcher using the system moved the map marker to direct the TurtleBot to 5 positions along a straight path, equally spaced at .47~m intervals. The path was traversed twice per trial by the TurtleBot and repeated over 10 trials. The \SystemName requested the TurtleBot's latest position every frame from the server API, starting a latency measurement on sending a request, and ending the measurement after updating the location indicator's position. A command measurement started when the map marker was placed and stopped once a response was received. A trajectory measurement also started on marker placement, and stopped once the computed path was received and all trajectory indicators were instantiated. We observed the location indicator has an average update latency of 170$\pm 0.14$~ms, and trajectory indicators have an average of 310$\pm 0.09$~ms. Trajectory indicators have higher latency because each path point must be transformed into the \SystemName's coordinate system and instantiated individually. For the command indicator, it took 1.52$\pm 1.55$~s for the TurtleBot to receive and respond to a command on average; although not ideal, we find in Sec.~\ref{sec:studyeval} that users did not mention this delay, and generally find the experience to be responsive.


% \vspace{-0.3cm}
\begin{table}[]
\centering
\caption{Performance for 3 obstructed real-world targets at varying distances, horizontal offsets, and angular offsets.}
% \scalebox{0.6}{%
\setlength{\tabcolsep}{2.5pt}
\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{llccccccccccccc}
\toprule
\multirow{2}{*}{Target} & \multirow{2}{*}{Metric (\%)} & \multicolumn{4}{c}{Distance (m)} & \multicolumn{4}{c}{Offset (cm)} & \multicolumn{3}{c}{Angle (°)} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-13}
& & 1.2 & 1.8 & 3 & 3.65 & 10 & 15.2 & 25.4 & 30.5 & 15 & 45 & 60 \\
\midrule
\multirow{3}{*}{Monitor} & \ObsPipeName Accuracy $\uparrow$            & 100 & 100 & 100 & 100 & 99 & 99 & 78 & 72 & 99 & 100 & 88 \\
                         & Failed detection $\downarrow$    & 0 & 0 & 0 & 0 & 1 & 0 & 22 & 28 & 1 & 0 & 12 \\
                         & False negative $\downarrow$      & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\
\midrule
\multirow{3}{*}{Plant}   & \ObsPipeName Accuracy $\uparrow$            & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 \\
                         & Failed detection $\downarrow$    & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
                         & False negative $\downarrow$      & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\midrule
\multirow{3}{*}{String} & \ObsPipeName Accuracy $\uparrow$  & 100 & 100 & 0 & 0 & 100 & 100 & 100 & 100 & 100 & 100 & 99 \\
                                   & Failed detection $\downarrow$  & 0 & 0 & 100 & 99 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
                                   & False negative $\downarrow$  & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule
\end{tabular}
}
\label{obstructedcaseresults}
\end{table}






% \vspace{0.05cm}
\subsection{\ObsPipeName Evaluation}
\label{subsec:odmsystemeval}

To evaluate the accuracy and scalability 
of the \ObsPipeName, we collected 100 performance measurements across multiple objects and a text string with the HoloLens in a variety of poses, with the headset at an equal height to the targets. We used a monitor and potted plant as object targets, and a 9-character label ("ITMkscT5o") as the text target. We ensured the YOLO output was accurate for the objects; text output was not verified, as all text is considered important regardless of content. For each target, we recorded accuracy, false negative and failed detection rates under known obstruction by a generic Unity cube. We collected data 
at 4 distances (1.2-3.65~m), 
4 horizontal offsets (10-30.5~cm), and 3 angular offsets (15–60°) to reflect realistic views. Here, failed detection percentage is the ratio of measurements in which YOLO or the OCR model failed to detect a target. The results are summarized in Table~\ref{obstructedcaseresults}.

For the text string, the \ObsPipeName performed well at distances of 1.2 and 1.8~m, with 100\% accuracy in both cases. This accuracy was maintained when the horizontal offset and angular offset of the HoloLens was varied. However, greater distances, the accuracy dropped dramatically to 0\%, almost entirely due to failed detections. The accuracies for the monitor and potted plant remained high with increasing distance. The performance on the potted plant was also good when horizontal and angular offsets were varied. Performance on the monitor degraded with these offsets however, dropping as low as 72\% accuracy for the horizontal offsets, and 88\% accuracy for the angular offsets. We suspect the high accuracy on the potted plant as compared to the monitor is the result of the plant's rotational symmetry, which the monitor lacks, along with the more featureless surface of the monitor. In nearly all cases, we found that accuracy degradations were the result of failed detections. Despite the performance degradation on text at greater distances, we show in our user study that the \ObsPipeName was effective in mitigating text obstructions. In future work, we will improve its ability to detect text that is farther from the camera.

We also characterize the latency of the \ObsPipeName, in a scenario with 2 real-world objects employed in our user study (a box label and a stuffed animal) and between 1 and 12 virtual cubes in the HoloLens's view, with 100 measurements per setting. 
%and investigate its scalability subject to the number of active virtual items (VIs). These VIs are 10×10×10~cm Unity cubes arranged in an even grid as their number increases. We performed 100 measurements of the round-trip latency starting with 1 VI, increasing up to 12 VIs. Measurements were taken with the HoloLens facing a blank wall with 1 box label and a stuffed animal object used in our user study in front of it. 
The \ObsPipeName achieves an average latency of 334$\pm 0.07$~ms with 1 VI in view, which increases by 3.8\%, to 347$\pm 0.12$~ms, with 12 VIs in view. The primary latency bottleneck was the OCR model, which required 110~ms to process an image on average; in future work, this could be remedied by employing a more computationally efficient OCR model. The relatively small increase in latency with the increased number of VIs suggests that the \ObsPipeName is well-suited for situations with a large number of VIs as there might be in AR-HRC contexts. %Even so, from these results, we find the \ObsPipeName is capable with increasing amounts of virtual content. 

%We also characterize the latency of the \ObsPipeName and investigate its scalability subject to the number of active virtual items (VIs). These VIs are 10×10×10~cm Unity cubes arranged in an even grid as their number increases. We performed 100 measurements of the round-trip latency starting with 1 VI, increasing up to 12 VIs. Measurements were taken with the HoloLens facing a blank wall with 1 box label and a stuffed animal object used in our user study in front of it. The \ObsPipeName achieves an average latency of 334$\pm 0.07$~ms with 1 VI in view, which increases to 347$\pm 0.12$~ms with 12 VIs in view. Deeper investigation into these latencies revealed the primary bottleneck was the OCR model, which required 110~ms to process an image on average. We suspect this could be remedied with a more optimized OCR model. Even so, from these results, we find the \ObsPipeName is capable with increasing amounts of virtual content. 

